Efficient linear scaling mapping for permutation symmetric Fock spaces

Numerically solving a second quantised many-body model in the permutation symmetric Fock space can be challenging for two reasons: (i) an increased complication in the calculations of the matrix elements of various operators, and (ii) a poor scaling of the cost of these calculations with the Fock space size. We present a method that solves both these problems. We find a mapping that can be used to simplify the calculations of the matrix elements. The mapping is directly generated so its computational cost scales only linearly with the space size and is negligible even for large enough sizes that approach the thermodynamic limit. A fortran implementation of the method as a library - FockMap - is provided along with a test program.

==> fockmap/README <==



##########################################################################
                          Instructions
##########################################################################

Two Steps:

1. Compile the library to obtain fockmap.a 
2. Compile the test program that uses fockmap.a 

These two steps are briefly explained below.

--------------------------------------------------------------------------
                       1. Compilation of the library
--------------------------------------------------------------------------

FockMap uses a makefile for its compilation. Edit Makefile in "fockmap/src/" 
if you like to change the compiler. On the command line, go to the source directory 
"fockmap/src/" and run "make" to compile the library. This will produce the 
library archive "fockmap.a" and also copy it to the test program directory
"fockmap/test/"

--------------------------------------------------------------------------
                      2. Compilation of the test program
--------------------------------------------------------------------------

Edit makefile "fockmap/test/Makefile" if you like to change the compiler. 
On the command line, go to the source directory "fockmap/test/" and 
run "make" to compile the program. This will produce the executable "test"
that can be run to test the library routines. To see the usage of the 
library routines, please see the source file for the test program 
"fockmap/test/main.f".

##########################################################################








##########################################################################
                        Directory Structure
##########################################################################

- source files of the library and its makefile are in the directory "fockmap/src/"
- source file for the test program and its makefile in the directory "fockmap/test/"

                    fockmap
                      |
                     / \
                  src   test
                  /      \
library source files      test program source files

--------------------------------------------------------------------------
              library source files in "fockmap/src/"
--------------------------------------------------------------------------

mapping.f:
Calculates the mapping.

mapn2.f:
Calculates the mapping for N=2 case.

triangles.f:
Calculates the triangular regions of the mapping.

basis.f:
Calculates the number of permutations, and the occupation frequencies for N-1,N modes.

basisall.f:
Calculates the number of permutations, and the occupation frequencies for 0,1,...,N modes

ratios.f:
Calculates the rations of the normalisation factors of the pair of permutation symmetric states for N-1 and N modes that are linked to each other via the mapping.

ratiosall.f:
Calculates the rations of the normalisation factors of the pair of permutation symmetric states for p-1 and p modes (p=1,...,N-1) that are linked to each other via the mapping.

factorial.f: 
Contains the factorial function.

binomial.f: 
Contains the binomial function.

sizes.f: 
Calculate the sizes of permutation symmetric subspaces for 0,1,...,N modes.

Makefile:
makefile for the library.


--------------------------------------------------------------------------
              test program in "fockmap/test/"
--------------------------------------------------------------------------


main.f:
Illustrates and tests calls to various library routines

Makefile:
makefile for the test program.

##########################################################################







==> fockmap/src/Makefile <==
##################################
# makefile: fockmap
##################################

FC 	= gfortran
FFLAGS= -O3 -g

SRC = factorial.f  binomial.f mapping.f mapn2.f  triangles.f \
 sizes.f basisall.f basis.f ratiosall.f ratios.f  

OBJ = $(SRC:.f=.o)

.SUFFIXES: .o .f

fockmap.a: $(OBJ)
	ar cr fockmap.a $(OBJ)
	cp fockmap.a ../test/.

.f.o: 
	$(FC) $(FFLAGS) -c $< -o $@

clean:
	rm -rf *.o fockmap.a
  

